Digital Contact Tracing Solutions: Promises, Pitfalls and Challenges

The COVID-19 pandemic has caused many countries to deploy novel digital contact tracing (DCT) systems to boost the efficiency of manual tracing of infection chains. In this paper, we systematically analyze DCT solutions and categorize them based on their design approaches and architectures. We analyze them with regard to effectiveness, security, privacy, and ethical aspects and compare prominent solutions with regard to these requirements. In particular, we discuss the shortcomings of the Google and Apple Exposure Notification API (GAEN) that is currently widely adopted all over the world. We find that the security and privacy of GAEN have considerable deficiencies as it can be compromised by severe, large-scale attacks. We also discuss other proposed approaches for contact tracing, including our proposal TRACECORONA, that are based on Diffie-Hellman (DH) key exchange and aim at tackling shortcomings of existing solutions. Our extensive analysis shows thatTRACECORONA fulfills the above security requirements better than deployed state-of-the-art approaches. We have implementedTRACECORONA, and its beta test version has been used by more than 2000 users without any major functional problems, demonstrating that there are no technical reasons requiring to make compromises with regard to the requirements of DCTapproaches.

==> sections/adversary.tex <==
%!TEX root=../tc.tex

We consider the adversary model and various requirements posed on the design of the tracing scheme. 
\todo{the following must be completely rewritten and contain sections for security and a section for privacy} 
\subsection{Security}

\noindent 
\textbf{\aFakeInfection} 
\label{sec:fake-infection}
The adversary is a malicious user \advUser that aims to lie about its infection state such that it can upload its encounter token information resulting in false exposure notifications for other users who have encountered \advUser. This is a serious attack because it affects the core functionality of the system and increases the demand for COVID-19 test.   

\paragraph{Attack's description}
The adversary \advUser tries to circumvent infection state verification, e.g., by colluding with the infected users to get infection state certificates.  

\paragraph{Adversary's capabilities}
The adversary \advUser has full control of its devices and CT apps. \advUser knows CT protocols.



\subsection{\aFakeExposure} 
\label{sec:fake-exposure}

\paragraph{Adversary's goal} The adversary is a malicious user \advUser that aims to circumvent the token matching protocol to generate fake exposure notifications. The motivation of this attack could be threefold: (1) it harms the reliability of the system, (2) a user can use it as an excuse to stay at home instead of going to work or participating in events, and (3) \advUser can intentionally share wrong encounter data to epidemiologists, thus sabotaging their analysis of the epidemiological situation.

\paragraph{Adversary's capabilities} the same as \aFakeInfection


\subsection{\aExploitingData} 
\label{sec:exploit-user-data}

\paragraph{Adversary's goal}
The adversary is a malicious user or a third party that aim to extract information of the users that is published.

\paragraph{Adversary's capabilities} the same as \aFakeInfection



\subsection{\aSurveillance}   
\label{sec:surveillance}

\paragraph{Adversary's goal}
The adversary is a malicious server \advServer that aims to collect and link data of users to profile them, extract social graphs or to track the users \cite{dp3tPeppptSecurity}. 


\paragraph{Adversary's capabilities}
The adversary \advServer has full control of the server and can access all the data store on the server.



\subsection{\aRelayAttack}
\label{sec:relay-attack}

\paragraph{Adversary's goal}
A relay adversary so-called wormhole adversary \advWormhole is an attacker that aims to inject fake contacts resulting in many false exposure notifications \cite{baumgartner2020mind,vaudenay2020analysis, crocker2020challenge}.

\paragraph{Attack's description}
The \advWormhole captures and relies short-range Bluetooth beacons from one place to other (distant) places such that two user Apps in two different locations, e.g., different cities, falsely think the beacon originates from a device in vicinity, i.e., within Bluetooth signal range. Adversary \advWormhole can relay Bluetooth messages like ephemeral IDs of users between distant devices so that the corresponding tracing apps falsely record encounter information even though the devices are not in proximity at the time of the encounter. \advWormhole can scale its attack by collecting ephemeral IDs from a location with a high infection rate (e.g., near COVID-19 test centers or a location known to suffer from a COVID-19 outbreak) and replay them to many other crowded places like shopping centers or railway stations in big cities. In this sense, \advWormhole creates a \emph{wormhole} to collect and spreads ephemeral IDs.

\paragraph{Adversary's capabilities}
The adversary has at least two devices that can capture and emit Bluetooth signals (i.e., ephemeral IDs) and Internet connection to forward the ephemeral IDs. It is trivial since existing attacks show that it can be done by using a US \$10-device e.g., \cite{Iovino2020timetravel}.  
 


\subsection{\aProfilingAttack}
\label{sec:profiling-attack}

\paragraph{Adversary's goal}
The adversary is an eavesdropper \advEavesdropper aims to track or profile users (using so-called profiling attacks), e.g., to perform surveillance of individual users.

\paragraph{Attack's description}
Since contact tracing apps constantly emit information into their surroundings, \advEavesdropper can deploy a Bluetooth sensor network to collect (sniff) ephemeral IDs to possibly track the movements of users.

\paragraph{Adversary's capabilities}
The adversary can install observation nodes. It is possible, e.g., Baumgärtner et al. \cite{baumgartner2020mind} demonstrate the adversary can use commercially available and inexpensive Bluetooth sensors.   


\subsection{\aMassSurveillance}
\label{sec:mass-surveillance}

\paragraph{Adversary's goal}
In this attack, a powerful adversary, malicious server colluding eavesdropper, aims to maximize the effectiveness of profiling attacks by linking the data that the malicious server \advServer has and the ephemeral IDs that the eavesdropper \advEavesdropper has collected.

\paragraph{Adversary's capabilities}
The adversary \advServer has full control of the server and can access all the data store on the server. Moreover, the adversary can deploy a Bluetooth sensor network to capture ephemeral broadcasted by CT apps.  
  






